MTV: Visual Analytics for Detecting, Investigating, and Annotating Anomalies in Multivariate Time Series

Detecting anomalies in time-varying multivariate data is crucial in various industries for the predictive maintenance of equipment. Numerous machine learning (ML) algorithms have been proposed to support automated anomaly identification. However, a significant amount of human knowledge is still required to interpret, analyze, and calibrate the results of automated analysis. This paper investigates current practices used to detect and investigate anomalies in time series data in industrial contexts and identifies corresponding needs. Through iterative design and working with nine experts from two industry domains (aerospace and energy), we characterize six design elements required for a successful visualization system that supports effective detection, investigation, and annotation of time series anomalies. We summarize an ideal human-AI collaboration workflow that streamlines the process and supports efficient and collaborative analysis. We introduce MTV (Multivariate Time Series Visualization), a visual analytics system to support such workflow. The system incorporates a set of novel visualization and interaction designs to support multi-faceted time series exploration, efficient in-situ anomaly annotation, and insight communication. Two user studies, one with 6 spacecraft experts (with routine anomaly analysis tasks) and one with 25 general end-users (without such tasks), are conducted to demonstrate the effectiveness and usefulness of MTV.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> tables/RQ.tex <==
\begin{table}[!htpb]
\begin{tabularx}{\linewidth}{@{}l >{\raggedright\arraybackslash}X@{}}
\toprule
\textbf{Participant}  & \textbf{Research Question}    \\ 
\midrule
General User
& \textbf{RQ1.}
Are they able to use \name~to perform anomaly investigation and annotation collaboratively?
\\
& \textbf{RQ2.}
How is their user experience using \name?
\\\\[-1.5ex]
% \midrule
Domain Expert
& \textbf{RQ3.}            
Is \name~ effective and efficient for performing their routine anomaly analysis tasks?
\\
% & \textbf{RQ4.}
% Does the investigation workflow cover all the scenarios?
% \\


\bottomrule
\end{tabularx}
\caption{ \label{tb:myRQ}
The research questions we aim to answer through the two user studies with general users and domain experts, respectively.
}
\end{table}

==> tables/functionalities.tex <==
\begin{table}[!htb]
\begin{tabularx}{\linewidth}{@{} l >{\raggedrigth\arraybackslash}X @{}}
\toprule
Functionality & Definition\\
\midrule
View Multiple Time Series & View multiple signals together at the same time\\
Periodic View & View a summarization of events through time \\
Multi-aggregation View & View the signal in multiple aggregation, e.g., 1 hour, 30 minutes etc.\\
Annotate Event & Assign a tag to an event based on its characteristics as well as add, delete, modify an event.\\
Discussion & Allow multiple user interaction through discussion and comments\\
Shape Search & Search for segments that are similar to a particular event \\
Composition & Compose cards to explore the analysis of multiple signalruns (experiments)\\
\bottomrule
\end{tabularx}
\end{table}

==> tables/glossary.tex <==
\begin{table}[ht]
    \centering
    \begin{tabular}{c|c|c}
    \toprule
      term          &  change   & definition   \\
    \midrule
      $\mathbf{x}$  &           & time series (vector) $\mathbf{x} = [\mathbf{x}^1, \mathbf{x}^2, \dots, \mathbf{x}^T]$\\
      $T$           &           & length of the time series\\
      $X$           &           & training dataset\\
      $N$           &           &  Number of training samples\\
      $x_i$         &           &  data point in $\mathbf{x}$ at time $i$\\
      $t$           &           &  window size\\
      $s$           &           &  step size\\
      $A$           &           &  vector of anomaly scores\\
      $\tau$        &           &  set of anomaly intervals\\
      $(t_s, t_e)$  &           &  anomaly interval starts at $t_s$ and ends at $t_e$\\
      $C$           &           &  set of candidate anomaly intervals identified by shape matching\\
    \bottomrule
    \end{tabular}
    \caption{Glossary}
    \label{tab:glossary}
\end{table}

==> tables/platform.tex <==
\begin{table}[!htb]
\begin{tabularx}{\linewidth}{@{} X *{7}{>{\centering\arraybackslash}p{0.1\linewidth}} @{}}
\toprule
&  \multicolumn{7}{c}{Functionality} \\
\cmidrule{2-8}
Platform & View Multiple Time Series & Periodic View & Multi-aggregation View & Annotate Event & Discussions & Shape Search & Compo\-sition\\
\midrule
Xu et al.  2020~\cite{xu2019clouddet} & \Checkmark & \Checkmark & \cellcolor{gray!20!white} & \Checkmark & \cellcolor{gray!20!white} & \cellcolor{gray!20!white} & \cellcolor{gray!20!white}\\
Alsallakh et al. 2014~\cite{alsallakh2014visual} & \Checkmark &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\Checkmark &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} \\
Sarkar et al. 2016~\cite{sarkar2016visual} &\Checkmark &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\Checkmark &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white}\\
Cao et al. 2016~\cite{cao2015targetvue} &\Checkmark &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\Checkmark &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white}\\
Xie et al. 2018~\cite{xie2018visual} & \cellcolor{gray!20!white} & \cellcolor{gray!20!white} & \cellcolor{gray!20!white} & \Checkmark & \cellcolor{gray!20!white} & \cellcolor{gray!20!white} & \cellcolor{gray!20!white}\\
Bernard et al. 2017~\cite{bernard2017visual} &  \cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\Checkmark &	\cellcolor{gray!20!white}\\
Cao et al. 2018~\cite{cao2017voila} & \cellcolor{gray!20!white} &	\cellcolor{gray!20!white} & \cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white} &	\cellcolor{gray!20!white}\\
\bottomrule
\end{tabularx}
\caption{Qwerty.}
\end{table}


==> texfiles/12.problem.tex <==
% \newcommand{\mathbf{A}}{\mathrm{T}}

\section{Study Context: Time Series Anomaly Detection}
\label{sec:context}
An anomaly detection task requires an input sequence $\mathbf{x} = [\mathbf{x}^1, \mathbf{x}^2, \dots, \mathbf{x}^T]$, which we refer to as a time series of length $T$. 
Each data point $\mathbf{x}^i \in \mathbb{R}^m$ is a vector that represents a multi-channel measurement. 
To simplify our notation, we use $m=1$ (i.e., $x^i \in \mathbb{R}$) where $x^i$ is now a scalar. 
This notation follows the definition of a single-variate time series; however, the same process can be extrapolated to represent multivariate time series when $\mathbf{x}^i \in \mathbb{R}^m$. 

Let us define an interval of timestamps as ($t_s, t_e$), where $t_s, t_e \in [1, T]$ and $t_s \leq t_e$. 
The objective of an anomaly detection task is to find intervals that are suspected to be anomalous. 
Formally, we denote the output as an anomaly set $\mathbf{A}$ where $\mathbf{A} = \{(t_j, t_{j+w}) \:|\: 1 \leq j < T - w\}$ and $w$ resembles the anomalous window width. 
In our definition, $w$ differs in each anomalous interval.
For example, for $\mathbf{x}= [x^1, x^2, x^3, x^4, \dots, x^T]$ and assuming that the following data points $x^2, x^3, x^4$ are anomalous points, then $\mathbf{A} = \{(t^2, t^4)\}$ is the output of the anomaly detection process (note $w = 3$ in this example). 

In this work, we use unsupervised learning models to identify anomalies.
Unsupervised learning is a common approach for anomaly detection within time series, due to a lack of labeled data and shifting contexts that change what is considered an anomaly -- a dataset labeled in one context may not apply to the new context at hand.
For the rest of the paper, we will use "time series" and "signals" interchangeably to represent time-varying variables based on the context.


==> texfiles/4.system_tech_detailed_version.tex <==
%!TEX root = ../main.tex
% !TeX spellcheck = en_US


\section{MTV}\label{sec:system}
\label{sec:mtv}

In this section, we first describe our approach of identifying anomalies through an end-to-end machine learning pipeline.
Next, we detail how to use shape-matching techniques to enhance annotating efficiency.
Finally, we describe the visual design of our system.

\subsection{Identifying anomalies with the end-to-end ML pipeline }

\begin{figure}[!htbp]
	\centering
	\includegraphics[width=1\linewidth]{figures/ml_pipeline2.pdf}
	\caption{The end-to-end ML pipeline for multivariate time series anomaly detection. (Top) The pipeline takes multiple signals as inputs and generates a list of intervals of timestamps ($t_s$, $t_e$) which are suspected to be anomalous. (Bottom) the pipeline is composed of 6 primitives, each serving one particular function.}
	\label{fig:ml_pipeline}
% 	\vspace{-3ex}
\end{figure}

Detecting anomalies within time series data does not simply mean training a prediction/reconstruction model. Numerous pre-processing and post-processing steps should be applied as well.
Fig.~\ref{fig:ml_pipeline} describes an entire ML pipeline from start to finish. 
At a high level, the pipeline takes multiple signals as inputs and generates a list of intervals of timestamps ($t_s$, $t_e$) which are suspected to \mbox{be anomalous (T1).}

A primitive is a reusable, self-contained, software component for machine learning~\cite{smith2020machine}. MTV's ML pipeline contains 6 fundamental primitives, each serving a particular function (Fig.~\ref{fig:ml_pipeline} Bottom), and each with various hyperparameters, the settings of which influence the ML outputs. Because domain experts generally do not have ML expertise, we have discussed with them what they hope to observe, and provide them with control through the landing page (Section~\ref{sec:landing_page}).


\textbf{Data pre-processing.}
The first two primitives transform the data into a clean format $\mathbf{x} = [x^1, x^2, \dots, x^T]$, where the interval between  $x^{t-1}$ and $x^{t}$ is equal and missing values are imputed with predefined strategies. The third primitive prepares a collection of training samples using a sliding window sequence approach.
For a window of size $t$ and step size $s$, we generate $N$ subsequences $X = \{x_{i}^{1\dots t}\}_{i=1}^N$, where $N = (T - t)/ s$.

\textbf{Modeling.}
The fourth primitive learns a prediction/reconstruction model to generate a predicted/reconstructed time series $\hat{\mathbf{x}}$. 
We identify the need to use different algorithms in different scenarios while collaborating with domain experts.
~\name~ has integrated three popular models, including a GAN-based model (TadGAN~\cite{geiger2020tadgan}), long short-term memory (LSTM~\cite{hundman2018detecting}), and autoregressive integrated moving average (Arima~\cite{pena2013anomaly}).

Each algorithm has its own benefits~\cite{geiger2020tadgan}: the GAN model performs well at handling complex signal data with myriad fluctuations; LSTM is a well-established sequence learning method suitable for many general scenarios; and Arima is a statistical model proven to work excellently when time series have remarkable trend and periodical patterns.
Bearing this high-level knowledge in mind, MTV allows users to choose ML outputs that apply the most suitable model for further investigation (Section~\ref{sec:landing_page}).

\textbf{Finding anomalies.}
Then, the fifth primitive computes the discrepancies between $\mathbf{x}$ and $\hat{\mathbf{x}}$ to locate potential anomalies, under the logic that higher discrepancies suggest a higher chance that the segment is anomalous. In other words, we generate $\mathbf{E} = [e^1, e^2, \dots, e^T]$ that measures the difference at every time step. Then we apply an exponentially weighted moving average (EWMA) on it, obtaining the smoothed error as below: 
\begin{equation}
\mathbf{E_s} = [e^{1}_s, e^{2}_s, \dots, e^{T}_s]
\label{eq:errors}
\end{equation}
The last primitive takes this error sequence as an input and computes a threshold. Any values regarding the
smoothed errors above the threshold are considered to be anomalies.
The threshold is selected from the set: 
$\bm{\theta} = \mu(\bm{e}_s) + k\sigma(\bm{e}_s)$
where $\mu$ and $\sigma$ denote the mean and standard deviation respectively. 
%%%% easy language %%%%
Eventually, $\theta$ is determined by finding a threshold that would bring about the maximum percent decrease in the mean and standard deviation of $\bm{e}_s$ if all error values above the threshold are eliminated~\cite{hundman2018detecting}. Now each anomalous sequence $\bm{e}_{seq}$ (continuous sequences of $e^{i}_s$ with the value above $\theta$) can be assigned a severity score $s$:
\begin{equation}
s = \frac{max(\bm{e}_{seq}) - \theta}{\mu(\bm{e}_s) + \sigma(\bm{e}_s)}
\label{eq:score}
\end{equation}
Now we can represent each anomalous sequence $\bm{e}_{seq}$ in the format of ($t_s, t_e$, $s$), where $t_s$ is the starting time of this sequence, $t_e$ is the ending time, and $s$ is the assigned severity score.

\subsection{Enhance annotating efficiency with shape -matching}
\label{sec:shape_matching}
\label{sec:mtv_shape_matching}
Due to the large-scale nature of the data, analysts are only able to annotate a limited number of events. 
We use the idea of ``shape-matching'' to enhance annotating efficiency (R4), as well as to improve the performance of the ML pipeline (R1).

We introduce a novel shape-matching algorithm for efficient shape search within time series data. We perform shape-matching in a signal-based manner.
The output of the shape-matching algorithm produces a set of candidate shapes in a signal $\mathbf{x}$ that are similar to a particular sub-sequence $\mathbf{s}$, under the constraint that the returned segments will not overlap with each other or any \mbox{existing events}. 

We adopt a sliding window approach to generate subsequences of $\mathbf{x}$, then compare them to $\mathbf{s}$ through a similarity measure $f(\cdot, \cdot)$.
We chose $f$ to be the total cost of finding the optimal mapping between two sequences, using either Euclidean or dynamic time warping (DTW~\cite{berndt1994using}) as the similarity measurement. The Euclidean method tends to find exactly matched shapes while DTW can tolerate a certain level of shifting. 

The full algorithmic process is described in the following pseudo-code (algorithm~\ref{alg:shape-matching}).
At each checkpoint $t_c$ we attempt to include the current most similar shape $\mathbf{c}$ in the candidate subset.
Prior to that, we check whether or not $\mathbf{c}$ overlaps with a preexisting candidate shape; if so, we keep the most similar between the two.
This procedure will return a set of non-overlapping candidate shapes $C$ that are most similar to $\mathbf{s}$.

\begin{algorithm}[!htb]
   \caption{Shape Matching}
   \label{alg:shape-matching}
    \begin{algorithmic}[1]
       \STATE {\bfseries Input:} Signal $\mathbf{x} = [x^1, x^2, \dots, x^T]$
       \STATE Sub-Sequence $\mathbf{s} = [s^{k+1}, s^{k+2}, \dots, s^{k+t}] $ where $ 1 \leq k < (T-t)$.
       \STATE {\bfseries Output:} Candidate sub-sequences $C$.
       \STATE Initialize $\mathbf{c} = \texttt{None}$ \hfill \texttt{// to hold candidate shape}
       \STATE Initialize $t_c = t$.
       \FOR{$i=1$ {\bfseries to} $T-t$}
       \STATE $\Tilde{\mathbf{x}} = [x^i, x^{i+1}, \dots, x^{i+t}]$ \hfill \texttt{// subsequence of $\mathbf{x}$}
       \IF{$f(\Tilde{\mathbf{x}}, \mathbf{s}) < f(\mathbf{c}, \mathbf{s})$}
       \STATE $\mathbf{c} \gets \Tilde{\mathbf{x}}$ \hfill \texttt{// update $\mathbf{c}$ to hold a more similar shape}
       \ENDIF
       \IF{$i > t_c$} 
       \IF{$C \cap \{\mathbf{c}\} \neq \phi$}
       \STATE $\mathbf{v} \gets C \cap \{\mathbf{c}\}$ \hfill \texttt{// overlapping sequence}
       \STATE $\mathbf{c} \gets \texttt{argmin} \: [f(\mathbf{c}, \mathbf{s}), f(\mathbf{v}, \mathbf{s})]$ \hfill \texttt{// keep most similar}
       \ENDIF
       \STATE $C = C \cup \{c\}$ \hfill\texttt{// add candidate shape}
       \STATE $\mathbf{c} = \texttt{None}$ \hfill \texttt{// reset}
       \STATE $t_c = t_c + t$
       \ENDIF
       \ENDFOR
       \STATE \textbf{return} $C$
    \end{algorithmic}
\end{algorithm}

We argue for three main uses for shape-matching (described below), all of which greatly enhance annotating efficiency and make anomaly investigation and annotations feasible for large-scale data.

\textbf{Annotation sharing.} 
Once the expert confirms that an annotated sequence is indeed an anomaly, s/he will be inclined to search for other segments that have not yet been flagged, but are similar to the confirmed event.
These similar segments are likely to receive the same annotations as the confirmed one.  

Fig.~\ref{fig:6657}b shows the selected event (b1) and its similar segments (b2 and b3). Analysts can quickly assign tags to them one after another or even all at once. (Fig.~\ref{fig:side_panels} Right).

\textbf{Decision support.} 
Sometimes the status of an anomaly is ambiguous, and choosing a proper tag is difficult. 
In this case, an expert can use shape-matching to find similar shapes (non-anomalous segments) to this event. By comparing the differences between them, analysts can quickly clarify why the anomaly detection algorithm identified this segment as anomalous. 

We introduce a superposed visualization in Section~\ref{sec:similar_segment_view} that allows for such comparisons. Fig.~\ref{fig:side_panels} (Right) shows one example, where the event under investigation can be compared to similar segments.  

\textbf{False alarm mitigation.}
After events have been properly annotated, we are able to mitigate false alarms (false positives) by leveraging the shape-matching algorithm. 
Consider an event that analysts may think is unworthy of exploration -- say, one tagged as ``Do not investigate'' or ``Normal'' (see details in Section.~\ref{sec:event_detail_view}). We can ask the system to prune existing events with the method described below.

We use the shape of one such event as a template to search a set of candidate similar shapes, which can be tuned according to a pre-defined threshold. Those supposedly anomalous segments identified by the ML pipeline are now pruned by checking whether they overlap with these candidate similar shapes, thus reducing the number of false positives.
%A similar strategy can be applied to mitigate false negatives by leveraging ``problem'' or ``previously seen'' tagged events.

==> texfiles/algorithm_sarah.tex <==
\section{Time Series Anomaly Detection and Similar Segment Search}\label{sec:algorithm}

\begin{table}[ht]
    \centering
    \begin{tabular}{c|c|c}
    \toprule
      term          &  change   & definition   \\
    \midrule
      $\mathbf{x}$  &           & time series (vector) $\mathbf{x} = [\mathbf{x}^1, \mathbf{x}^2, \dots, \mathbf{x}^T]$\\
      $T$           &           & length of the time series\\
      $X$           &           & training dataset\\
      $N$           &           &  Number of training samples\\
      $x_i$         &           &  data point in $\mathbf{x}$ at time $i$\\
      $t$           &           &  window size\\
      $s$           &           &  step size\\
      $A$           &           &  vector of anomaly scores\\
      $\tau$        &           &  set of anomaly intervals\\
      $(t_s, t_e)$  &           &  anomaly interval starts at $t_s$ and ends at $t_e$\\
      $C$           &           &  set of candidate anomaly intervals identified by shape matching\\
    \bottomrule
    \end{tabular}
    \caption{Glossary}
    \label{tab:glossary}
\end{table}


\textbf{Feeding back user annotations.}
Identifying anomalies is only one part of the problem, the more crucial aspect is to integrate the expert's feedback into the model.
After the model generates a collection of potential anomalies, we showcase them to the expert user, as ask them to annotate the presented segments.
We use the idea of ``shape matching'' to feed back the annotations from the user to improve the performance of the system.

In the remainder of this section, we describe our approach of identifying anomalies through adversarial learning. 
In addition, we detail our methodology in which we integrate back the user feedback through shape matching.


\subsection{Identifying Anomalies with Adversarial Learning}
We describe one of the approaches of using unsupervised learning, namely Generative Adversarial Network (GAN). 
We define the construction of this model in the ``TadGAN'' pipeline[add ref]. 
At a high level, the pipeline receives a signal input $\mathbf{x}$ and tries to reconstruct this signal which we denote as $\hat{\mathbf{x}}$. 
Then it computes the discrepancies between $\mathbf{x}$ and $\hat{\mathbf{x}}$ to locate the potential anomalies, the intuition being, higher discrepancies suggest a higher probability of the segment as being anomalous.

\subsubsection{Adversarial Training}
In reconstruction-based anomaly detection, we want to learn a model that can reconstruct signals that best depict the original signal.
We assume that the model will not be able to reconstruct anomalies as well as ``normal'' instances, due to the loss of information during reconstruction. 
This is not a trivial task given the high-dimensionality of the data as well as the temporal dynamics. 
We introduce a two mapping functions, namely, an encoding neural network $\mathcal{E}: X \rightarrow Z$ to reduce the dimension of the signal into its latent representation, and $\mathcal{G}: Z \rightarrow X$ that generates a signal based on $Z$ (i.e., maps it back into the high dimensional space).
Both $\mathcal{E}$ and $\mathcal{G}$ are implemented using long short-term memory cells (LSTM) to withhold information captured from the temporal dependencies. We measure their loss by the L2 norm objective.
\begin{equation*}
    V_{L2}(\mathcal{E}, \mathcal{G}) = \mathbb{E}_{x \sim \mathbb{P}_X} [\|x - \mathcal{G}(\mathcal{E}(x))\|]_2
\end{equation*}

Moreover, we introduce adversarial loss to both $\mathcal{E}$ and $\mathcal{G}$ [add ref and benefit of two discriminators]. They are supervised by two independent discriminators (``critics'') to indicate the realness of encoded, and generated signals, respectively.
\begin{align*}
    V_X(\mathcal{C}_x, \mathcal{G}) &= \mathbb{E}_{x \sim \mathbb{P}_X}[\mathcal{C}_x(x)] - \mathbb{E}_{z \sim \mathbb{P}_Z}[\mathcal{C}_x(\mathcal{G}(z))] \\
    V_Z(\mathcal{C}_z, \mathcal{E}) &= \mathbb{E}_{z \sim \mathbb{P}_Z}[\mathcal{C}_z(z)] - \mathbb{E}_{x \sim \mathbb{P}_X}[\mathcal{C}_z(\mathcal{E}(x))]
\end{align*}

Collectively, this generates our objective function for training our model:
\begin{equation}
    \label{eq:obj_gan}
    \min_{\mathcal{E}, \mathcal{G}} \max_{\mathcal{C}_x \in \: \mathbf{C}_x, \mathcal{C}_z \in \: \mathbf{C}_z} V_{L2}(\mathcal{E}, \mathcal{G}) + V_X(\mathcal{C}_x, \mathcal{G}) + V_Z(\mathcal{C}_z, \mathcal{E})
\end{equation}

Given a time series $\mathbf{x} = [x^1, x^2, \dots, x^T]$, we generate a collection of training samples by using a sliding window sequence approach. For a window of size $t$ and step size $s$, we generate $N$ sub-sequences $X = \{x_{i}^{1\dots t}\}_{i=1}^N$, where $N = (T - t)/ s$. In addition, we introduce $Z = \{z_{i}^{1\dots k}\}_{i=1}^N$ a set of randomly sampled segments from the normal distribution $z \sim \mathcal{N}(0, 1)$, where $k$ denotes the dimension of the latent space. We feed $X$ and $Z$ to our GAN model and train it with the objective defined in~\ref{eq:obj_gan}.

\subsubsection{Computing Errors}
Recall that $X$ is composed of $N$ sub-sequences, for each sequence $x_{i}$ of length $t$, we generate a reconstructed sequence of the same
length: $x_{i} \rightarrow \mathcal{E}(x_{i}) \rightarrow \mathcal{G}(\mathcal{E}(x_{i})) \approx \hat{x}_{i}$. 
In other words, we generate $\hat{X} = \{\hat{x}_{i}^{1\dots t}\}_{i=1}^N$.
Note that for each point in time $j$, there are multiple reconstructed values, to flatten ${\hat{X}}$ back into a signal $\mathbf{\hat{x}}$, we use the median of reconstructed values.  
From there, we suggest multiple approaches for comparing the real signal $\mathbf{x}$ with reconstructed signal $\mathbf{\hat{x}}$, which we define through $RE(\mathbf{x}, \mathbf{\hat{x}})$.

\paragraph{Point-wise Difference}. In this approach, we compute the reconstruction error as the discrete-point-wise difference between true and reconstructed values at each time step: $f(\mathbf{x}, \mathbf{\hat{x}}) = \sum_t^T |x^t - \hat{x}^t|$.

\paragraph{Area Difference}. In this approach, we compute the reconstruction error as the as the similarity between local regions.
It is defined as the average difference between the areas underneath two curves of length $l$: $RE(\mathbf{x}, \mathbf{\hat{x}}) = \sum_t^T \frac{1}{2 * l} | \int_{t - l}^{t + l} x^t - \hat{x}^t \; dx|$.
 
\paragraph{Dynamic Time Warping (DTW)}. In this approach, we take signal latency into consideration by finding the optimal many-to-many mapping between two given time sequences.
The optimal path $W^\ast$ between the two sequences is defined as the path that returns the minimum distance measure subject to the boundary conditions, as well as constraints on continuity and monotonicity. 
To find $W^\ast = (w_1, w_2, \dots, w_K)$ where $K$ is the length of the warp path and $T \leq K < 2 * T$  and $w_k = (i,j)$ is the $k^{th}$ element of that warp path mapping $x_i$ to $\hat{x}_j$. 
The optimal path is given by $RE(\mathbf{x}, \mathbf{\hat{x}}) = \min_W [\frac{1}{K} \sum_{k=1}^K \sqrt{w_k}]$.

In addition to reconstruction error, we leverage the score produced by critic $\mathcal{C}_x$ which distinguishes between real input sequences and synthetic ones. 
The output of $\mathcal{C}_x$ has a positive indication of the realness value where larger values denote real sequences and smaller ones illustrate fake sequence. 
Therefore, once the Critic is trained, it can directly serve as an anomaly measure for time series sequences.
We combine both errors to produce an overall error $\bm{e}_i = \alpha RE(x_i) + (1 - \alpha) \mathcal{C}_x(x_i)$.

From here, we can use sliding window to compute thresholds. 
The intuition behind windowing is the usage of historical error scores to evaluate the current threshold.
This approach is useful to identify contextual anomalies.
For each sliding window, points with errors larger than the threshold $\theta$ are considered anomalous $\bm{e}_a = \{e \in \bm{e} | e > \theta\}$.
Consequently, we can identify anomalous sequences as $\{\bm{e}^i_{seq} | i = 1, \dots, K\}$ where $\bm{e}^i_{seq} = (e_{start(i)}, e_{end(i)})$.
To compute $\theta$, we can use a simple static threshold defined as $k$ standard deviations from the mean of the window.
Alternatively, we can compute $\theta$ using dynamic thresholds.

\hlred{Anomaly scoring - lstm paper}

\subsubsection{Dynamic Thresholding}
The intuition is that exceptionally high errors could suggest some unexpected behaviors.
Thus, we borrow an unsupervised method by Hundman et al.~\cite{hundman2018detecting}, where an error threshold can be efficiently learned from error sequences without labeled data or statistical assumptions about errors.
To identify whether a point behaves abnormally at time step $i$, an error sequence $\bm{e} = [e^{i-h}, \cdots, e^{i-1}, e^{i}]$ is evaluated, where $h$ specify the number of historical errors.
To better capture the continuous anomalous time steps, we employ a simple moving average (ma) over the errors to get a smoothed set of errors:
%To better capture the continuous anomalous time steps, we employ exponentially-weighted moving average (EWMA)~\cite{hunter1986exponentially} to smooth the spikes in errors:
$$\bm{e}_s = \text{ma}(\bm{e}) = [e^{i-h}_s, \cdots, e^{i-1}_s, e^{i}_s]$$
%\dy{not work in air quality case, use simple smoothing}
%To avoid the situation that abrupt changes in values would lead to many sharp spikes in error values even the behavior is normal~\cite{shipmon2017time}, the error sequence is then smoothed with exponentially-weighted average (EWMA)~\cite{hunter1986exponentially}: $$\bm{e}_s = [e^{t-h}_s, \cdots, e^{t-1}_s, e^{t}_s]$$
The threshold is then selected from the set: $$\bm{\theta} = \mu(\bm{e}_s) + k\sigma(\bm{e}_s)$$
where $\mu$ and $\sigma$ denote the mean and standard deviation respectively and $k \in \mathbb{R}_0^+$  (one hyperparameter of this block and in practice, we often consider $k \in [0, 12]$).
Eventually, $\theta$ is determined by:
%\begin{equation}
$$\underset{\bm{\theta}}{argmax} \quad \frac{\Delta\mu(\bm{e}_s)/\mu(\bm{e}_s) + \Delta\sigma(\bm{e}_s)/\sigma(\bm{e}_s)}{|\bm{e}_a| + |\bm{E}_{seq}|^2}	$$
%\label{eq:piecewise_cpd}
%\end{equation}
where
\begin{align*} 
&\Delta\mu(\bm{e}_s) = \mu(\bm{e}_s)-\mu(\{e_s \in \bm{e}_s, | e_s < \theta\}) \\
&\Delta\sigma(\bm{e}_s) = \sigma(\bm{e}_s)-\sigma(\{e_s \in \bm{e}_s, | e_s < \theta\}) \\
&\bm{e}_a = \{e_s \in \bm{e}_s | e_s > \theta\} \\
&\bm{E}_{seq} = \text{continuous sequences of } e_a \in \bm{e}_a
\end{align*}

The intuition is that finding a threshold that would bring about the maximum percent decrease in the mean and standard deviation of $\bm{e}_s$ if all error values above the threshold are eliminated.
$\bm{E}_{seq}$ and $\bm{e}_a$ in the denominator are introduced as penalization terms to prevent having too many anomalous error values and sequences by simply choosing a very small threshold.
Now each anomalous sequence $\bm{e}_{seq} \in \bm{E}_{seq}$ can be assigned with an anomaly score $s$:
\begin{equation}
s = \frac{max(\bm{e}_{seq}) - \theta}{\mu(\bm{e}_s) + \sigma(\bm{e}_s)}
\label{eq:score}
\end{equation}


\begin{algorithm}[tb]
   \caption{Anomaly Detection Procedure}
   \label{alg:ad-procedure}
    \begin{algorithmic}
       \STATE {\bfseries Input:} Signal $\mathbf{x} = [x^1, x^2, \dots, x^T]$
       \STATE {\bfseries Output:} Anomaly Scores $\mathbf{A}$.
       \STATE Initialize $X$, window size $t$, and step size $s$.
       \FOR{$i=1$ {\bfseries to} $T$}
       \STATE $X \gets X \cup \{\mathbf{x}^{i:i+t}\}$
       \ENDFOR
       \STATE \texttt{train model on } $X$
       \FOR{$i=1$ {\bfseries to} $N$}
       \STATE $\hat{x}_{i} \gets \mathcal{G}(\mathcal{E}(x_{i}))$
       \STATE $RE(x_{i}) \gets f(x_{i}, \hat{x}_{i})$
       \STATE $\bm{e}_i \gets \alpha RE(x_{i}) + (1 - \alpha) \mathcal{C}_x(x_{i})$
       \ENDFOR
    \end{algorithmic}
\end{algorithm}

\subsection{Shape Matching (User Feedback)}
% how implement
% primary goal: to integrate our investigation workflow. (1) annotate event, they want to find similar events. tag is confirmed (2) we are not confirming the tag, but we want to find the similar segment to compare and figure out if its an anomaly or not (an aide to the expert). Investigate why it was identified as an anomaly but this one did. (3) filter the events to mitigate false positives and false negatives within.
% user feedback 

From a procedural aspect, the signal is passed to an anomaly detection task to produce anomalies. 
These anomalies are then presented to the expert user such that they can properly annotate them \textbf{(we will go over annotation in [add section])}.
We record the user interactions with the anomalies and integrate the annotations back into the system.
The objective is to allow the user to investigate similar events to the confirmed anomalies.

We introduce shape-matching, an algorithm for efficient shape search within time series data.
The objective of shape-matching is to increase the efficacy of anomaly detection identification. 
We view its usage in three folds:
\begin{itemize}
    \item \textit{Efficiency.} After the expert confirms the status of the anomaly, S/he is inclined to search for other segments that are similar to the confirmed event.
    \item \textit{Informative.} The status of the anomaly is still ambiguous, the user then uses shape-matching to gain more information about the shape and clarifies the reason why the anomaly detection algorithm identified this segment as anomalous. 
    \item \textit{Mitigation.} After the events are properly annotated, we mitigate false positives and false negatives by learning from the events' shapes.
\end{itemize}

\begin{algorithm}[tb]
   \caption{Shape Matching}
   \label{alg:shape-matching}
    \begin{algorithmic}[1]
       \STATE {\bfseries Input:} Signal $\mathbf{x} = [x_1, x_2, \dots, x_T]$
       \STATE Sub-Sequence $\mathbf{s} = [s_{k+1}, s_{k+2}, \dots, s_{k+t}] $ where $ 1 \leq k < (T-t)$.
       \STATE {\bfseries Output:} Candidate sub-sequences $C$.
       \STATE Initialize $\mathbf{c} = \texttt{None}$ \hspace{5pt} \texttt{// to hold candidate shape}
       \STATE Initialize $t_c = t$.
       \FOR{$i=1$ {\bfseries to} $T-t$}
       \STATE $\Tilde{\mathbf{x}} = [x_i, x_{i+1}, \dots, x_{i+t}]$ \hspace{5pt} \texttt{// subsequence of $\mathbf{x}$}
       \IF{$f(\Tilde{\mathbf{x}}, \mathbf{s}) < f(\mathbf{c}, \mathbf{s})$}
       \STATE $\mathbf{c} \gets \Tilde{\mathbf{x}}$ \hspace{5pt} \texttt{// update $\mathbf{c}$ to hold a more similar shape}
       \ENDIF
       \IF{$i > t_c$} 
       \IF{$C \cap \{\mathbf{c}\} \neq \phi$}
       \STATE $\mathbf{v} \gets C \cap \{\mathbf{c}\}$ \hspace{5pt} \texttt{// overlapping sequence}
       \STATE $\mathbf{c} \gets \texttt{argmin} \: [f(\mathbf{c}, \mathbf{s}), f(\mathbf{v}, \mathbf{s})]$ \hspace{5pt} \texttt{// keep most similar}
       \ENDIF
       \STATE $C = C \cup \{c\}$ \hspace{5pt} \texttt{// add candidate shape}
       \STATE $\mathbf{c} = \texttt{None}$ \hspace{5pt} \texttt{// reset}
       \STATE $t_c = t_c + t$
       \ENDIF
       \ENDFOR
       \STATE \textbf{return} $C$
    \end{algorithmic}
\end{algorithm}

We perform shape-matching on a signal-based manner, with a flexibility on which similarity metric to use.
The output of the shape matching algorithm is to produce a set of candidate shapes in a signal $\mathbf{x}$ that are similar to a particular sub-sequence $\mathbf{s}$.
We adopt a sliding window approach to generate sub-sequences of $\mathbf{x}$ then compare them to $\mathbf{s}$ through a similarity measure $f(\cdot, \cdot)$.
In our implementation, we chose $f$ to be the total cost of finding the optimal mapping between two sequences using DTW~\cite{berndt1994using}.
Other alternatives also present themselves, such as area under the curve or euclidean distance. 
At each checkpoint $t_c$ we attempt to include the current most similar shape $\mathbf{c}$ into the candidate subset.
But prior to that, we check whether or not $\mathbf{c}$ overlaps with a preexisting candidate shape, if so, keep the most similar between the two.
The result of this procedure will return a set of non-overlapping candidate shapes $C$ that are most similar to $\mathbf{s}$.


==> texfiles/goals_requirements.tex <==


%observations of machine learning and visualization techniques in practice over the past years, as well as our own experiences collaborating with domain experts from multiple industries and fields, 

\section{Design goals}
Our work with a number of experts whose daily work is to monitor signals from large systems (turbines, satellites, water pipelines) have enabled us to delineate a list of codified requirements for time series anomaly analysis at an industrial scale. Below we present these requirements and the design goals they led to and guided the development of MTV. A successful interface system must enable users to: 

\noindent \textbf{UR: Pull together relevant signals and data for analysis.} 
Machine learning can exhaust every possible hyperparameter combination and obtain meaningful results in different contexts. For example, using different levels of time granularity or a missing value imputing strategy to preprocess data will likely result in very different anomaly detection results. However, all the results make sense in certain analytical scenarios. With machine learning pipelines built across a wide number of signals, users typically want to have flexibility to create a grouping of signals that is pertaining to their domain and interest. 

\begin{itemize}
    \item \textbf{VIG: An intuitive way to compose a analytic dashboard for analysis}
\end{itemize}
    
    
\noindent \textbf{UR: Perform investigations \textit{in-situ}.} Users want to stay within the interface and perform all their investigations without having to switch between interfaces, data sources, other tools or software applications. This translated to three goals for the interface. 
    
\begin{itemize}
	\item \textbf{VIG: Offer intuitive visual interface for displaying, annotating and interacting with anomalies.}
	\\
	The visual interface should display when and where the anomalies occurred. Create, read (aka retrieve), update, and delete (CRUD) functions should be supported when analysts interact with an event.
	
	\item \textbf{VIG: Offer a workflow to share analysis}
	Furthermore, the system should allow analysts to document their thoughts, provide external contextual information, make annotations on  anomalous events, and explore annotations from other analysts. 
	
	\item \textbf{VIG: Enable multi-faceted and multi-granular visual explorations of time series.}
	\\
	%To interpret and annotate anomalies, the system should provide analysts with contextual information about them, allowing them to confirm or refute its conclusions.
	The ability to show time series patterns from different perspectives (trend, periodicity, etc.) and in different granularities (second, minute, hour, etc) is required. Investigations require looking at raw signals. 
    \end{itemize}
    
\noindent \textbf{UR: Inform ML and future investigations.} They would like to provide information that could be later used by machine learning to improve models, and share the results of their analysis and investigation with their peers in future. 
    \begin{itemize}
    \item \textbf{VIG: Store, track, record and feedback}: Interaction history should also be recorded and traceable through the interface. 
    \item \textbf{VIG: Facilitate efficient and intelligent anomaly identification.}: In addition, the system is expected to learn from human's interactions (e.g. tag/comment/edit/create/delete) with existing anomalous events to know how to intelligently point analysts to the most important segment of time series, prioritize them, and provide information about why they are important.
	\end{itemize}
   
 %   The scale of time series data is often overwhelming -- a significant concern for experts.
  
    %Given a very large time series, the system should support fast and robust automated anomaly detection. 
    
    \item[--] Be able to take part in any subpart of the investigative workflow. Not all users want to create new dashboards - some want to enhance investigations, add information to investigations, add events. 
    
\end{itemize}

%\begin{enumerate}[label=\textbf{G\arabic*}]

   % \item \textbf{Facilitate efficient and intelligent anomaly identification.}
   % \\
  %  The scale of time series data is often overwhelming -- a significant concern for experts.
    % To maintain a complex system such as spacecraft, over thousands of time-varying measurements  (e.g., temperature, radiation, and power) are being collected in a second/minute granularity.
   % Given a very large time series, the system should support fast and robust automated anomaly detection.
  %  In addition, the system is expected to learn from human's interactions (e.g. tag/comment/edit/create/delete) with existing anomalous events to know how to intelligently point analysts to the most important segment of time series, prioritize them, and provide information about why they are important.
    
   % \item \textbf{Provide the flexibility to interact with outputs from machine learning.}
    \\
   % 
   % Thus, the system should allow analysts to interact with outputs from machine learning to select what they want to investigate.
	
	
	
  %  \item \textbf{Follow an easy and streamlined workflow to perform anomaly analysis}
  %  \\
   % Mind stress to learn the tool for domain experts like Jean -> go linearly -> embed their workflow.
  %  [respond to their job not just for research]
   % [get into the real end-users]
  %  [the first-hand people]
    
%\end{enumerate}

==> texfiles/intro_old.tex <==
%!TEX root = ../main.tex
% !TeX spellcheck = en_US

\section{Introduction}\label{sec:introduction}
The rapid proliferation of sensors and connected devices has led to massive and increasing accumulation of temporal observation data (a.k.a. multivariate time series). As more and more industries rely on such data, detecting and analyzing anomalies in time series becomes increasingly important for critical use cases ranging from cyber-intrusion and fault detection to preventative maintenance and fraud prevention~\cite{ahmad2017unsupervised}. 

A time series anomaly is a time point or period during which a system exhibits unusual behavior. To efficiently detect such unusual behaviors in what are often enormous data sets, and ease the burden of the humans often tasked with such detection, a variety of automated anomaly detection methods using statistical or machine learning techniques have been proposed~\cite{hodge2004survey, chandola2009anomaly, goldstein2016comparative, habeeb2019real}.
In practice, however, the performance of these methods is restrained for the following three reasons.
%it is notoriously difficult to have these
%fully automated methods achieve ideal performance.
 
First, the frequent lack of labeled anomalies for learning and evaluating models leads to a bottleneck to high performance. Though many unsupervised or semi-supervised approaches have been explored, it is still easy to produce too many false positives, exacerbating the diagnosis burden placed on system maintainers. 
Second, many real-world systems are highly dynamic and contextually dependent, making it difficult to accurately define anomalies. Without a way to integrate human knowledge into the anomaly investigation workflow, many true anomalies may remain hidden.
Third, temporal data sets collected by sensors are often large and can suffer from quality issues such as inconsistent or missing formatting, making them substantially more difficult to analyze. 
Thus, we stress the necessity of developing a more scalable, reliable, and flexible human-plus-ML workflow to detect and investigate anomalies in multivariate time series. 

Data visualization can provide effective support for this workflow by integrating humans' valuable expertise and creativity into anomaly investigation via various visual representations of information and human-machine interactions~\cite{ware2019information}.
Recent years have witnessed increasing efforts to combine visualization and automated anomaly detection for time series data analysis~\cite{xu2019clouddet, xie2018visual}.

But visualizing multivariate time series analysis requires determining how to get across central aspects of the data: for instance, scalability (what is the right level of detail of time series data to show), multi-dimensionality (how many time series should be displayed), and interpretability (how best to represent the contextual information that helps determine legitimate anomalies). Other questions come up as well:
(1) \textbf{End-user:}
A large number of end users with the routine job of monitoring time series data may have minimal or no technical background. To help them, we must understand what they are hoping to \underline{\textit{observe}} or \underline{\textit{control}} about the data and the analysis process, and avoid using overly technical jargon or complicated visualizations. An intuitive visual design is required to alleviate users' learning burden.
(2) \textbf{Annotation:} 
From the user's point of view, it is the results' interpretation that matters. However, existing systems lack the crucial ability to document and share such interpretations, without which it may be difficult to translate results into real actionable decisions. We stress that the ability to annotate anomalies, as well as to organize and present these annotations, is a highly important part of any anomaly detection system.
(3) \textbf{Workflow:}
Recently, several unified visual analysis systems have been proposed for anomaly detection on temporal data~\cite{cao2017voila, xu2019clouddet, xu2018ecglens}. However, most of them are designed for particular applications, and failed to describe a unified workflow that can detect, investigate, and annotate anomalies systematically. 
%currently there exists no unified human-plus-ML workflow for multivariate time series data anomaly analysis. The workflow should ensure the analysis efficiency facing massive data and enable smooth interaction between humans and machines without introducing confusion. 

Awareness of these gaps comes through our collaboration with domain experts in the aerospace and energy industries, who spend a considerable amount of time monitoring telemetry data from large industrial devices in order to identify and analyze potential hazardous events. In cooperation with these experts, we have characterized the common design requirements necessary for a unified anomaly detection system that fully takes advantage of both the power of human intelligence and the computation capability of machines. We therefore propose MTV, a visual interactive system to support the detection, investigation, and annotation anomalies in large-scale multivariate time series data. 

The system employs an unsupervised method based on Generative Adversarial Networks to perform robust and effective time series anomaly detection. 
The system contains two pages: a) a landing page that shows the overview experiments done by automated methods; b) an analysis page where multiple coordinated views are adopted along with a set of novel visualization and interaction designs to facilitate multi-faceted exploration at different levels of granularity. In particular, the annotation overview and detail view are carefully designed to provide a good experience for annotation exploration and creation.
Furthermore, we summarize a streamlined and efficient human-plus-ML workflow to allow for efficient time series anomaly analysis. Finally, we present an evaluation of the system via user studies done with two types of potential end users -- domain experts and general data analysts.
    
% Our system adopts multiple coordinated views to allow users interact with time series data in various forms.

The main contributions of this work are as follows:
\begin{itemize}
    \item
    A comprehensive GAN-based visual analytics system for efficient anomaly detection, with several intuitive visualization and interaction designs integrated for multi-faceted and variously granular time series data exploration and anomaly investigation and annotation.
    \item
    A streamlined and efficient human-plus-ML workflow, which starts with users giving high-level input to machines, defining analysis tasks, and investigating and annotating anomalies, and ends with anomaly detectors learning from user annotations and adjusting detection strategies for future improvement.
    \item 
    A novel layout algorithm to optimize the order of small multiples to better display co-occurred anomalies (events that happened close together in time but in different signals/variables), and a novel similar time segments-searching algorithm to support the anomaly investigation workflow.
    \item
    A user study in which domain experts from the aerospace industry use spacecraft telemetry data to show the usefulness of MTV, and a usability study in which general end-users reveal the potential broad-scale benefits of such a system.       
\end{itemize}

The remainder of the paper is structured as follows.
Section~\ref{sec:relatedwork} discusses related work.
Section~\ref{sec:background} introduces our work with domain experts and summarizes the system design requirements.
Section~\ref{sec:algorithm} describes the machine learning algorithm we used for automated anomaly detection, as well as the shape-matching algorithm that plays an important role in anomaly investigation workflow. Visual designs are introduced in Section~\ref{sec:system}.
We present the system evaluations in Section~\ref{sec:evaluation} including the domain expert track and the general user track.
Finally, we conclude the paper and discuss potential future research directions in Section~\ref{sec:conclusion}.

